SAGMAN: Stability Analysis of Graph Neural Networks on the Manifolds

Modern graph neural networks (GNNs) can be sensitive to changes in the input graph structure and node features, potentially resulting in unpredictable behavior and degraded performance. In this work, we introduce a spectral framework known as SAGMAN for examining the stability of GNNs. This framework assesses the distance distortions that arise from the nonlinear mappings of GNNs between the input and output manifolds: when two nearby nodes on the input manifold are mapped (through a GNN model) to two distant ones on the output manifold, it implies a large distance distortion and thus a poor GNN stability. We propose a distance-preserving graph dimension reduction (GDR) approach that utilizes spectral graph embedding and probabilistic graphical models (PGMs) to create low-dimensional input/output graph-based manifolds for meaningful stability analysis. Our empirical evaluations show that SAGMAN effectively assesses the stability of each node when subjected to various edge or feature perturbations, offering a scalable approach for evaluating the stability of GNNs, extending to applications within recommendation systems. Furthermore, we illustrate its utility in downstream tasks, notably in enhancing GNN stability and facilitating adversarial targeted attacks.

==> Lipschitz_Constant_Calculation.tex <==
\subsection{Distance Mapping Distortions Calculation}
\label{Lipschitz}
The geodesic distance metric is the most intuitive choice to quantify the distance mapping distortion (DMD) for each sample on a low-dimensional manifold. However, the prevailing methods of calculating geodesic distance are computationally taxing\cite{naitzat2020topology} and even the most advanced randomized methods \cite{williams2014faster} do not alleviate this computational burden adequately. To circumvent this, we employ effective-resistance distances, which serve as an upper bound to the geodesic distance (a detailed proof is provided in Appendix \ref{Effective-resistance distance}). By computing the average DMD between node $p$ and all its adjacent nodes, we obtain the DMD score for node $p$. Subsequently, we can utilize the SPADE method\cite{cheng2021spade} to efficiently approximate the average DMD score for individual data samples:
\begin{equation}\label{formula_spade2}
SPADE^G(p)\propto\frac{1}{|\mathbb{N}_X(p)|}\sum_{q_i\in \mathbb{N}_X(p)}^{} \left(\delta^G(p, q_i)\right)^3.
\end{equation}
where $q_i \in \mathbb{N}_X(p)$ denotes the $i$-th neighbor of node $p$ in graph $G_X$, and $\mathbb{N}_X(p) \in V$ represents the set of nodes that includes all of $p$'s neighbors.
%When calculating the maximum distance mapping distortions $\delta^G_{max}$ using the effective-resistance distance, the SPADE score\cite{cheng2021spade} serves as an upper bound for $\delta^G_{max}$.
%\begin{equation}
%\label{spade_model_socre}
%SPADE^G \triangleq \lambda_{max}(L_Y^+ L_X) \ge K^* \ge \delta^G_{max}
%\end{equation}
%Equation \ref{spade_model_socre} suggests that the SPADE score also serves as an upper bound for the best Lipschitz constant $K^*$ within the manifold context. A higher SPADE score for a function (model) indicates reduced adversarial robustness, as the output becomes more sensitive to minor input perturbations. 



